Non-perturbative Renormalization of Improved Staggered Bilinears

We compute Z-factors for general staggered bilinears on fine (a \approx 0.09 fm) MILC ensembles using both asqtad and HYP-smeared valence actions, comparing the results to the predictions of one-loop perturbation theory. This is an extension of previous work on the coarse (a \approx 0.12 fm) MILC ensembles. It provides a laboratory for studying NPR methodology in the staggered context, and is an important stepping stone for fully non-perturbative matching factors in ongoing computations of B_K and other weak matrix elements. We also implement non-exceptional RI/SMOM renormalization conditions using the asqtad action and present first results.

==> figs/HYP_ratios_both.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,6480.00)%
      \csname LTb\endcsname%
      \put(3600,6260){\makebox(0,0){\strut{}HYP-smeared Bilinears}}%
    \gplgaddtomacro\gplbacktext{%
      \put(946,720){\makebox(0,0)[r]{\strut{}0.94}}%
      \put(946,1280){\makebox(0,0)[r]{\strut{}0.96}}%
      \put(946,1840){\makebox(0,0)[r]{\strut{}0.98}}%
      \put(946,2400){\makebox(0,0)[r]{\strut{}1.00}}%
      \put(946,2960){\makebox(0,0)[r]{\strut{}1.02}}%
      \put(946,3519){\makebox(0,0)[r]{\strut{}1.04}}%
      \put(946,4079){\makebox(0,0)[r]{\strut{}1.06}}%
      \put(946,4639){\makebox(0,0)[r]{\strut{}1.08}}%
      \put(946,5199){\makebox(0,0)[r]{\strut{}1.10}}%
      \put(946,5759){\makebox(0,0)[r]{\strut{}1.12}}%
      \put(2092,220){\makebox(0,0){\strut{}V}}%
      \put(2498,220){\makebox(0,0){\strut{}A}}%
      \put(3918,220){\makebox(0,0){\strut{}T}}%
      \put(176,3239){\makebox(0,0){\Large $\frac{Z_{\gamma_S \otimes \xi_F}}{Z_{\gamma_S \otimes \mathbf{1}}}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \put(4346,5866){\makebox(0,0){\strut{}$\hash$ links:}}%
      \csname LTb\endcsname%
      \put(4349,5646){\makebox(0,0)[r]{\strut{}zero}}%
      \csname LTb\endcsname%
      \put(4349,5426){\makebox(0,0)[r]{\strut{}one}}%
      \csname LTb\endcsname%
      \put(4349,5206){\makebox(0,0)[r]{\strut{}two}}%
      \csname LTb\endcsname%
      \put(4349,4986){\makebox(0,0)[r]{\strut{}three}}%
      \csname LTb\endcsname%
      \put(4349,4766){\makebox(0,0)[r]{\strut{}four}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(6300,220){\makebox(0,0){\strut{}S}}%
      \put(7331,440){\makebox(0,0)[l]{\strut{}1.05}}%
      \put(7331,1373){\makebox(0,0)[l]{\strut{}1.10}}%
      \put(7331,2306){\makebox(0,0)[l]{\strut{}1.15}}%
      \put(7331,3240){\makebox(0,0)[l]{\strut{}1.20}}%
      \put(7331,4173){\makebox(0,0)[l]{\strut{}1.25}}%
      \put(7331,5106){\makebox(0,0)[l]{\strut{}1.30}}%
      \put(7331,6039){\makebox(0,0)[l]{\strut{}1.35}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{HYP_ratios_both}}%
    \gplfronttext
  \end{picture}%
\endgroup

